Dithered backprop: A sparse and quantized backpropagation algorithm for more efficient deep neural network training

Deep Neural Networks are successful but highly computationally expensive learning systems. One of the main sources of time and energy drains is the well known backpropagation (backprop) algorithm, which roughly accounts for 2/3 of the computational complexity of training. In this work we propose a method for reducing the computational cost of backprop, which we named dithered backprop. It consists in applying a stochastic quantization scheme to intermediate results of the method. The particular quantisation scheme, called non-subtractive dither (NSD), induces sparsity which can be exploited by computing efficient sparse matrix multiplications. Experiments on popular image classification tasks show that it induces 92% sparsity on average across a wide set of models at no or negligible accuracy drop in comparison to state-of-the-art approaches, thus significantly reducing the computational complexity of the backward pass. Moreover, we show that our method is fully compatible to state-of-the-art training methods that reduce the bit-precision of training down to 8-bits, as such being able to further reduce the computational requirements. Finally we discuss and show potential benefits of applying dithered backprop in a distributed training setting, where both communication as well as compute efficiency may increase simultaneously with the number of participant nodes.

==> preliminaries.tex <==
\section{Preliminaries}
Quantization is the projection of numbers from a set with mostly real values to a smaller set of discrete values. These values are called \textit{quantization points}. It is a tool that has been used widely in signal processing and data encoding. For instance, analog-to-digital conversions of audio-signals make use of a particular quantization called \textit{Uniform quantization}. It rounds the given values in such a way that the quantization points get evenly distributed in the input space. A \textit{mid-tread} uniform quantization function is defined as follows: 
\begin{equation}
y = Q(x) = \Delta \floor{\frac{x}{\Delta} + \frac{1}{2}}
\end{equation}
where $x$ is an \textit{input signal}, $\Delta$ the \textit{quantization step size} and $\floor{}$ the \textit{floor} operation returning the greatest integer smaller or equal to its argument. The quantization stepsize  determines the distance between adjacent quantization points. 
The resulting quantization error is then defined as the difference of the system output and the system input:
\begin{equation}
\epsilon = y - x = Q(x) - x
\end{equation}
Deterministic quantization functions like this one result in a deterministic quantization error that is fully dependent on the input signal. There is a deterministic mapping from the distinct input signals to their corresponding quantization errors, resulting in a biased quantization function. 
However, a uniform quantization system with additive dither signal, also called \textit{non-subtractive dither} (NSD), does not suffer from the that limitation. It is defined by:
\begin{equation}
y = Q(x+\nu) = \Delta \floor{\frac{x+\nu}{\Delta} + \frac{1}{2}}
\label{eq:NSD}
\end{equation}
where $\nu$ is a \textit{dither noise} which is drawn from a probability distribution with probability density function (pdf) $p_{\nu}$.
The dither noise $\nu$ is injected in order to make the quantization \textit{unbiased}. Dither noise signals have in general the function to randomize quantization funtions. It allows to model quantizations as random variables and hence to investigate their statistical moments.
\subsection{Appropriate Dither Distributions}
According to \cite{lipshitz_quantization_1992}, in order to decouple the first $m$ moments of the quantization error of a uniform quantization system with NSD from the system input, the dither signal has to be drawn from a distribution that fulfills the following condition:
\begin{equation}
P_{\nu}^{(i)}  \left( \frac{k}{\Delta} \right) = 0   \quad  \forall k \in \mathbb{Z}_0 \quad \textrm{and} \quad i = 0, 1, ..., m - 1
\label{eq:approp_dist}
\end{equation}
with $\Delta$ being the quantization step size, $P_{\nu}$ the characteristic function (cf) of the dither signal, i.e. the Fouri	er transform of its pdf $p_{\nu}$, and $P_{\nu}^{(i)}$ its $i$-th derivative. Furthermore, it was shown that when the above condition is fulfilled for a particular value of $m$, the first $m$ moments of the quantization error are given by
\begin{equation}
\mathbb{E}[\epsilon^m] = \sum_{l=0}^{\floor{\frac{m}{2}}}
{m\choose{2l}} {\left(\frac{\Delta}{2}\right)}^{2l} \frac{\mathbb{E}[{\nu}^{m-2l}]}{2l + 1}
\end{equation}
which results in the following equations for the first two moments:
\begin{equation}
\mathbb{E}[\epsilon] = \mathbb{E}[\nu] ,
\label{eq:first_moment}
\end{equation}
\begin{equation}
\mathbb{E}[\epsilon^2] = \mathbb{E}[{\nu}^2] + \frac{\Delta^2}{12} 
\label{eq:second_moment}
\end{equation}
As we can see, using an appropriate dither signal, the moments of the quantization error are directly determined by the moments of the dither signal. This allows us to control the error moments by the choice of dither signal. Moreover, for dither signals that fulfill the above condition for $m$ $\ge$ max$(m_1 , m_2)$, one can derive a general equation for the joint error moments $\mathbb{E}[\epsilon_1^{m_1} \epsilon_2^{m_2}]$, which is given in \cite{lipshitz_quantization_1992}. More importantly, if this dither signal is sampled independently the joint error moments are uncorrelated:
\begin{equation}
\mathbb{E}[\epsilon^{m_1} \epsilon^{m_2}] = \mathbb{E}[\epsilon^{m_1}] \mathbb{E}[\epsilon^{m_2}] 
\end{equation}\\
Thus, using an independently sampled dither signal that fulfills the condition from
above for $m$ $\ge$ 1, the quantization error of distinct input samples is uncorrelated:
\begin{equation}
\begin{split}
cov(\epsilon_1, \epsilon_2) &= \mathbb{E}[\epsilon_1 \epsilon_2] - \mathbb{E}[\epsilon_1] \mathbb{E}[\epsilon_2]\\
&= \mathbb{E}^2[\epsilon] - \mathbb{E}^2[\epsilon]\\
&= 0
\end{split}
\end{equation}  
%\subsection{Triangular Dither}
%\label{sec:triangular_dither}
%We refer to a dither signal that is independently sampled from a triangular pdf with a mean of zero and an amplitude of $2\Delta$ as \textit{triangular dither}. It can be shown that using such a dither distribution fulfills the condition from equation \ref{eq:approp_dist} for $m=2$ and thus renders the first two moments of the quantization error independent from the input signal. Furthermore, as shown by \cite{wannamaker_theory_2000}, it is the only dither signal that fulfills this condition while minimizing the second moment of the quantization error. Therefore, triangular dither is an optimal choice for input-independent error mean and variance.\\
%We can sample from such a triangular dither distribution by summing two independent random samples from a rectangular pdf, each with a mean of zero and an amplitude of $\Delta$.
%\begin{equation}
%	\nu = \nu_1 + \nu_2 \quad \mathit{with} \quad \nu_1, \nu_2 \sim \mathcal{U}(-\frac{\Delta}{2}, \frac{\Delta}{2}).
%\end{equation}
%Since a uniform distribution $\mathcal{U}(-a, a)$ has second moment $\frac{(2a)^2}{12}$, the triangular dither signal has second
%moment
%\begin{equation}
%	\mathbb{E}[\nu^2] = \mathbb{E}[\nu_1^2] + \mathbb{E}[\nu_2^2] = \frac{\Delta^2}{6}
%\end{equation}
%and using equations \ref{eq:first_moment} and \ref{eq:second_moment} we can show that the resulting quantization error has
%first and second moment
%\begin{equation}
%	\mathbb{E}[\epsilon] = 0,
%\end{equation}
%\begin{equation}
%\mathbb{E}[\epsilon^2] = \frac{\Delta}{4}.
%\end{equation}
\subsection{Uniform Dither}
\label{sec:uniform_dither}
We refer to a dither signal that is independently sampled from a rectangular pdf with a mean of zero and an amplitude of $\Delta$ as uniform dither.  Uniform dither, as described here, fulfills the condition in equation \ref{eq:approp_dist} for $m=1$ and thus only renders the first moment of the quantization error independent from the input. Therefore, the variance of the quantization error is still dependent on the input and thus not directly controllable by the choice of quantization step size, as it is the case for triangular dither. However, we found that the variance of the quantization error that results from using a uniform dither signal is bounded by the error variance that results from using triangular dither, which used a triangular pdf instead of a rectangular. We summarize this finding in the following conjecture which we verify experimentally in appendix B.1.\\
\\
\textbf{Conjecture}. \textit{Let Q be a mid-tread uniform quantization function with quantization step size $\Delta$}	
\begin{equation}
	Q(x) = \Delta [\frac{x}{\Delta} + \frac{1}{2}],
\end{equation}
\textit{and $\nu$ a random variable that follows a uniform distribution with a mean of zero and amplitude equal to the quantization step size}
\begin{equation}
	\nu \sim \mathcal{U}(-\frac{\Delta}{2}, \frac{\Delta}{2}).
\end{equation}
\textit{Then, the quantization error of a uniform quantization system with non-subtractive dither}
\begin{equation}
	\epsilon = Q(x+\nu) - x
\end{equation}
\textit{has a second moment bounded by}
\begin{equation}
	\mathbb{E}[\epsilon^2] \le \frac{\Delta^2}{4}.
\end{equation}
As stated by the conjecture above, given the same quantization step size, the variance of the quantization error induced by uniform dither is less than or equal to the quantization error induced by triangular dither. However, the noise that is actually induced has input-dependent variance - the noise is modulated. Instead of controlling the exact variance of the induced noise, we can only control the upper bound of the variance. This is a disadvantage since our desired quantization scheme should have controllable error variance such that the method can adapt to a required noise scale for the resulting parameter gradients. However, input-dependent noise variance during the back propagation algorithm, could also represent a helpful pre-conditioning of the noise regarding the training procedure. The primary objective, though, remains to induce sparsity in order to save calculations.
\subsubsection{Induced Sparsity}
The output sparsity of a dithered uniform quantization scheme is dependent on the input and the dither distributions. In order to analyze the output sparsity of a dithered uniform quantization system, we first have to formalize the distribution of the values that are being quantized. These values consist of the system inputs and the dither samples:
\begin{equation}
s = x + \nu
\end{equation}
\begin{equation}
y = Q(s)
\end{equation}
To describe the sparsity of the output $y$ we first need to define the pdf of $s$. Since, the
value of $s$ is given by the sum of two random variables, its pdf is the convolution of the
summand pdfs:
\begin{equation}
\begin{split}
f_s(s)	&= (f_x * f_{\nu})(s) \\
&= \int_{-\infty}^{\infty} f_x(s=-\tau)f_v(\tau) d_{\tau}
\end{split}
\end{equation} \\
where $f_{\nu}$ is the pdf of the dither signal which is defined as
\begin{equation}
f_{\nu_u}(t) = 
\begin{cases}
\frac{1}{\Delta} &\quad \mathrm{if} - \frac{\Delta}{2} \le t \le \frac{\Delta}{2} \\
0 &\quad \mathrm{otherwise}.
\end{cases}
\end{equation}
for the uniform dither.\\
Then, since due to the rounding operations all values of $s$ in the interval $[−\frac{\Delta}{2}, \frac{\Delta}{2})$ are quantized to zero, we can define the probability of an output value
being zero based on the probability density of $s$ as follows:
\begin{equation}
p(y = 0) = \int_{-\frac{\Delta}{2}}^{\frac{\Delta}{2}} f_s(s)ds.
\label{eq:31sp}
\end{equation}
In order to evaluate the impact of the dither signal on the induced sparsity, we make some assumptions about the input pdf $f_x$. Pre-activation gradients (in networks using ReLU activation) are distributed according to a zero-centered Laplace-like distribution. Then, approximation of the distribution of pre-activation gradients by fitting a Laplace distribution allows us to determine the induced sparsity, by solving equation \ref{eq:31sp} after $\Delta$.

